Hidden in Plain Sight: an Empirical Study about The Instruction Stacks of Coding Agents

Coding agents send their models more than the user's prompt: they add instructions, tool definitions, and environmental context that form an instruction stack. This stack guides execution and changes across releases, yet remains largely unexposed to users and insufficiently characterized in research. We present a longitudinal, cross-agent study of the instruction stacks captured in the first model requests of 1,886 releases of Claude Code, Codex, Gemini CLI, Qwen Code, and OpenCode. Under controlled conditions, we analyze their composition and evolution and trace changes in the four open-source agents to documented motivations. Our findings show why examining the system prompt or reporting the model alone provides an incomplete account of agent inputs. Tool definitions dominate three agents' latest requests, while occasional concentrated revisions alter instructions governing tool use, attribution, and coding style. Such revisions can complicate how researchers identify agent-authored contributions and interpret generated code. We also found that only 48% of examined change units directly explain the motivation for stack revisions. Across agents, shared capabilities emerge despite increasingly distinct wording. These findings expose an evolving, incompletely documented layer of agent design. The findings motivate documenting captured instruction stacks alongside agent releases, models, and user prompts, and preserving the rationale behind their revisions.

==> figures/table-adoption.tex <==
% Generated by scripts/rq4/make-charts.py. Do not edit.
\multicolumn{6}{@{}l}{\emph{Tool categories}} \\
Shell execution & \checkmark & \checkmark & -- & \checkmark & -- \\
File reading & \checkmark & Aug'25 & \checkmark & \checkmark & \checkmark \\
File editing & \checkmark & -- & -- & \checkmark & -- \\
Code search & (\checkmark) & -- & \checkmark & \checkmark & \checkmark \\
Web access & Mar'25 & Jan'26 & \checkmark & \checkmark & \checkmark \\
Planning & (Apr'25) & Oct'25 & Nov'25 & \checkmark & Sep'25 \\
Subagent delegation & \checkmark & Mar'26 & Nov'25 & Jun'25 & Sep'25 \\
Memory & -- & -- & (\checkmark) & -- & (\checkmark) \\
Extension loading & Sep'25 & (Oct'25) & (Jan'26) & Dec'25 & Feb'26 \\
User questions & (Dec'25) & Feb'26 & (Feb'26) & (Jan'26) & (Mar'26) \\
\midrule
\multicolumn{6}{@{}l}{\emph{Codes}} \\
\code{context management} & \checkmark & \checkmark & Oct'25 & (\checkmark) & Sep'25 \\
\code{memory} & \checkmark & -- & \checkmark & (\checkmark) & \checkmark \\
\code{execution policy} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{tool guidance} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{communication guidance} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{engineering guidance} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{role and scope} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{capability catalog} & \checkmark & Dec'25 & \checkmark & Jun'25 & \checkmark \\
\code{identity} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
\code{context facts} & \checkmark & May'25 & \checkmark & \checkmark & \checkmark \\
\code{scaffolding} & Jan'26 & (May'25) & \checkmark & Dec'25 & \checkmark \\


==> figures/table-agreement.tex <==
% Generated by scripts/rq1/make-charts.py. Do not edit.
\code{context management} & 198 & 0.52 & 0.79 \\
\code{memory} & 402 & 0.95 & 0.98 \\
\code{execution policy} & 581 & 0.62 & 0.89 \\
\code{tool guidance} & 2{,}869 & 0.76 & 0.94 \\
\code{communication guidance} & 4{,}585 & 0.83 & 0.94 \\
\code{engineering guidance} & 1{,}641 & 0.71 & 0.90 \\
\code{role and scope} & 976 & 0.67 & 0.85 \\
\addlinespace[2pt]
\code{capability catalog} & 309 & 0.25 & 0.96 \\
\code{identity} & 216 & 0.84 & 0.94 \\
\code{context facts} & 954 & 0.71 & 0.86 \\
\addlinespace[2pt]
\code{scaffolding} & 64 & 0.71 & 0.91 \\
\addlinespace[2pt]
\code{unresolved} & 1 & 0.22 & 1.00 \\
\midrule
All codes & 12{,}796 & 0.75 & 0.92 \\
Families & 12{,}796 & 0.70 & 0.91 \\


==> figures/table-code-change.tex <==
% Generated by scripts/rq2/make-charts.py. Do not edit.
\code{context management} & +0.2 & \cellcolor[HTML]{dbe8f8}+0.4 & \cellcolor[HTML]{86b6ef}+2.8 & $-$0.2 & \cellcolor[HTML]{dbe8f8}+0.8 \\
\code{memory} & \cellcolor[HTML]{dbe8f8}+1.0 & 0 & \cellcolor[HTML]{86b6ef}+2.7 & $-$0.2 & \cellcolor[HTML]{3987e5}\color{white}+3.8 \\
\code{execution policy} & +0.1 & \cellcolor[HTML]{dbe8f8}+0.3 & +0.1 & \cellcolor[HTML]{dbe8f8}+0.5 & \cellcolor[HTML]{86b6ef}+3.4 \\
\code{tool guidance} & \cellcolor[HTML]{f6d6d3}$-$0.3 & \cellcolor[HTML]{3987e5}\color{white}+4.2 & \cellcolor[HTML]{3987e5}\color{white}+6.4 & \cellcolor[HTML]{efb3ad}$-$2.3 & \cellcolor[HTML]{3987e5}\color{white}+4.3 \\
\code{communication guidance} & \cellcolor[HTML]{efb3ad}$-$1.6 & \cellcolor[HTML]{3987e5}\color{white}+8.5 & \cellcolor[HTML]{e34948}\color{white}$-$5.3 & \cellcolor[HTML]{f6d6d3}$-$0.9 & \cellcolor[HTML]{dbe8f8}+0.5 \\
\code{engineering guidance} & \cellcolor[HTML]{efb3ad}$-$1.5 & \cellcolor[HTML]{b7d3f6}+2.1 & \cellcolor[HTML]{dbe8f8}+0.8 & \cellcolor[HTML]{dbe8f8}+0.6 & \cellcolor[HTML]{e68b84}$-$2.5 \\
\code{role and scope} & \cellcolor[HTML]{dbe8f8}+1.2 & \cellcolor[HTML]{dbe8f8}+0.7 & \cellcolor[HTML]{b7d3f6}+2.2 & \cellcolor[HTML]{f6d6d3}$-$0.6 & \cellcolor[HTML]{dbe8f8}+0.9 \\
\addlinespace[2pt]
\code{capability catalog} & \cellcolor[HTML]{3987e5}\color{white}+5.6 & \cellcolor[HTML]{b7d3f6}+2.3 & \cellcolor[HTML]{86b6ef}+2.9 & \cellcolor[HTML]{dbe8f8}+0.6 & \cellcolor[HTML]{3987e5}\color{white}+4.0 \\
\code{identity} & \cellcolor[HTML]{dbe8f8}+0.4 & $-$0.2 & +0.2 & +0.2 & +0.1 \\
\code{context facts} & 0 & \cellcolor[HTML]{dbe8f8}+1.1 & \cellcolor[HTML]{dbe8f8}+0.6 & +0.2 & \cellcolor[HTML]{dbe8f8}+0.5 \\
\addlinespace[2pt]
Tool definitions & +36.3 & +17.4 & $-$1.7 & $-$6.7 & +81.0 \\


==> figures/table-documentation.tex <==
% Generated by scripts/rq3/make-charts.py. Do not edit.
Codex & 106 & 6 & 33 & 48 & 19 & 49 & 99 & 1 & 0 \\
Gemini CLI & 119 & 1 & 62 & 32 & 6 & 75 & 40 & 40 & 19 \\
OpenCode & 133 & 49 & 45 & 37 & 18 & 48 & 75 & 17 & 7 \\
Qwen Code & 138 & 0 & 49 & 51 & 1 & 64 & 58 & 40 & 2 \\
\midrule
Total & 496 & 56 & 48 & 42 & 10 & 57 & 66 & 27 & 7 \\


==> figures/table-motivation-codes.tex <==
% Generated by scripts/rq3/make-charts.py. Do not edit.
\code{context management} & 119 & 43 & \cellcolor[HTML]{aeada4}30 & \cellcolor[HTML]{aeada4}30 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{d0cfc7}19 & \cellcolor[HTML]{dddcd5}14 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{c3c2b7}28 & \cellcolor[HTML]{dddcd5}14 \\
\code{memory} & 295 & 15 & \cellcolor[HTML]{68675f}\color{white}53 & \cellcolor[HTML]{dddcd5}13 & 0 & \cellcolor[HTML]{9a9990}40 & \cellcolor[HTML]{d0cfc7}20 & \cellcolor[HTML]{c3c2b7}27 & \cellcolor[HTML]{dddcd5}13 & 0 \\
\code{execution policy} & 137 & 24 & \cellcolor[HTML]{68675f}\color{white}54 & \cellcolor[HTML]{e9e8e3}8 & \cellcolor[HTML]{e9e8e3}8 & \cellcolor[HTML]{e9e8e3}8 & \cellcolor[HTML]{c3c2b7}25 & \cellcolor[HTML]{e9e8e3}4 & \cellcolor[HTML]{dddcd5}12 & \cellcolor[HTML]{dddcd5}12 \\
\code{tool guidance} & 1{,}206 & 94 & \cellcolor[HTML]{807f78}\color{white}44 & \cellcolor[HTML]{d0cfc7}21 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{d0cfc7}22 & \cellcolor[HTML]{dddcd5}11 & \cellcolor[HTML]{e9e8e3}5 & \cellcolor[HTML]{dddcd5}15 & \cellcolor[HTML]{d0cfc7}19 \\
\code{communication guidance} & 1{,}313 & 58 & \cellcolor[HTML]{68675f}\color{white}52 & \cellcolor[HTML]{dddcd5}10 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{dddcd5}14 & \cellcolor[HTML]{dddcd5}10 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{d0cfc7}19 & \cellcolor[HTML]{d0cfc7}21 \\
\code{engineering guidance} & 865 & 57 & \cellcolor[HTML]{68675f}\color{white}53 & \cellcolor[HTML]{dddcd5}12 & 0 & \cellcolor[HTML]{dddcd5}12 & \cellcolor[HTML]{e9e8e3}9 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{d0cfc7}19 & \cellcolor[HTML]{dddcd5}16 \\
\code{role and scope} & 429 & 42 & \cellcolor[HTML]{68675f}\color{white}52 & \cellcolor[HTML]{dddcd5}12 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{d0cfc7}17 & \cellcolor[HTML]{d0cfc7}17 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{dddcd5}14 & \cellcolor[HTML]{e9e8e3}10 \\
\addlinespace[2pt]
\code{capability catalog} & 491 & 59 & \cellcolor[HTML]{aeada4}31 & \cellcolor[HTML]{d0cfc7}20 & \cellcolor[HTML]{f4f3f0}2 & \cellcolor[HTML]{807f78}\color{white}49 & \cellcolor[HTML]{e9e8e3}5 & \cellcolor[HTML]{e9e8e3}3 & \cellcolor[HTML]{dddcd5}12 & \cellcolor[HTML]{e9e8e3}7 \\
\code{identity} & 48 & 14 & \cellcolor[HTML]{aeada4}36 & \cellcolor[HTML]{dddcd5}14 & 0 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{c3c2b7}29 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{c3c2b7}29 & 0 \\
\code{context facts} & 261 & 56 & \cellcolor[HTML]{9a9990}39 & \cellcolor[HTML]{dddcd5}14 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{c3c2b7}25 & \cellcolor[HTML]{e9e8e3}7 & \cellcolor[HTML]{e9e8e3}9 & \cellcolor[HTML]{aeada4}30 & \cellcolor[HTML]{e9e8e3}9 \\
\addlinespace[2pt]
\code{scaffolding} & 23 & 8 & \cellcolor[HTML]{9a9990}38 & \cellcolor[HTML]{c3c2b7}25 & 0 & 0 & 0 & 0 & \cellcolor[HTML]{68675f}\color{white}50 & 0 \\
\addlinespace[2pt]
Tool definitions & 487 & 294 & \cellcolor[HTML]{c3c2b7}26 & \cellcolor[HTML]{dddcd5}12 & \cellcolor[HTML]{f4f3f0}3 & \cellcolor[HTML]{aeada4}31 & \cellcolor[HTML]{e9e8e3}6 & \cellcolor[HTML]{e9e8e3}5 & \cellcolor[HTML]{c3c2b7}25 & \cellcolor[HTML]{dddcd5}11 \\


==> figures/table-placement.tex <==
% Generated by scripts/rq1/make-charts.py. Do not edit.
Claude Code & 2.1.243 & 493 & \cellcolor[HTML]{aeada4}60.4 & \cellcolor[HTML]{d0cfc7}37.7 & -- & \cellcolor[HTML]{f4f3f0}1.9 \\
Codex & 0.149.1 & 174 & \cellcolor[HTML]{68675f}\color{white}85.6 & -- & \cellcolor[HTML]{e9e8e3}12.7 & \cellcolor[HTML]{f4f3f0}1.7 \\
Gemini CLI & 0.56.0 & 192 & \cellcolor[HTML]{52514e}\color{white}98.6 & -- & -- & \cellcolor[HTML]{f4f3f0}1.4 \\
OpenCode & 1.18.22 & 907 & -- & 0 & \cellcolor[HTML]{52514e}\color{white}100.0 & $<$0.1 \\
Qwen Code & 0.22.0 & 120 & -- & \cellcolor[HTML]{68675f}\color{white}86.1 & -- & \cellcolor[HTML]{e9e8e3}13.9 \\


==> figures/table-rq3.tex <==
% Generated by scripts/rq3/make-charts.py. Do not edit.
Codex & 174 & 158 & 172 & 65 & 155 & 61 & 145 \\
Gemini CLI & 192 & 186 & 191 & 111 & 180 & 107 & 102 \\
OpenCode & 907 & 882 & 894 & 119 & 853 & 119 & 112 \\
Qwen Code & 120 & 119 & 119 & 65 & 118 & 64 & 86 \\
\midrule
Total & 1{,}393 & 1{,}345 & 1{,}376 & 360 & 1{,}306 & 351 & 445 \\


==> figures/table-segment-change.tex <==
% Generated by scripts/rq2/make-charts.py. Do not edit.
Claude Code & 253 (51.5) & 656 & 630 & 162 & 69 & 57 & 47 & 356 \\
Codex & 63 (36.6) & 412 & 206 & 77 & 52 & 18 & 9 & 40 \\
Gemini CLI & 56 (29.3) & 326 & 254 & 81 & 4 & 15 & 15 & 51 \\
OpenCode & 107 (12.0) & 1{,}145 & 1{,}279 & 118 & 158 & 22 & 26 & 146 \\
Qwen Code & 65 (54.6) & 569 & 382 & 99 & 81 & 65 & 15 & 74 \\
\midrule
Total & 544 (29.1) & 3{,}108 & 2{,}751 & 537 & 364 & 177 & 112 & 667 \\

